A change-of-coordinates from Geometry to Algebra, applied to Brick Tilings

A proof is sketched of the Polynomial Conjecture of the author (circulated as preprint "Brick Tiling and Monotone Boolean Functions", available at the http://www.math.ufl.edu/~squash/tilingstuff.html url) which says that the family of minimal tilable-boxes grows polynomially with dimension. An important ingredient of the argument is translating the problem from its finite-dimensional geometric framework to the algebraic setting of an infinite-dimensional lattice.

==> everytex.tex <==
%%%%%%%%%%%%%%%% Done in every Tex file %%%%%%%%%%%%%%%%

\ifx\everytexLoaded\relax\endinput
\else\global\let\everytexLoaded\relax\fi

	%%% Experimental %%
%!
% \def\makeactive#1{\catcode`#1 = \active \ignorespaces}%
% 
% \def\access{\catcode`\@=11}	% This macro does NOT seem to work!
% 			   	% (In the context of using \font@.)
%  \def\endaccess{\catcode`\@=\active}  %! Use of this may get me into
%    % trouble since the \catcode of \@ may not be RESTORED to what
%    % it was.  Look in the new amstex for a correct version of this.



%%% New %%%
% The \cn was moved from stylechanges.ams.tex.
\define\cn#1{\finalinfo{cn:\,\sl#1}}
\define\mathrev#1{\finalinfo{{\sl M\!R:}\,\bf#1}} %15Jul1998


			%%%%%% PRINTING
\def\ManualFeed{\special{!statusdict /manualfeed true put}}
\def\Landscape{\special{landscape}}

			%%%%%% EMACS DEPENDENT STUFF
\let\group=\begingroup	% so that my TeX-insert-endTHING function, works.

\def\glet{\global\let}
\def\messageln{\immediate\write16 }
\let\endcomment=\relax

  % Font related stuff (PERMANENT MEANING)
\font\zapften =pzcmi at 10pt % ZapfChancery-MediumItalic 
\font\zapffifteen =pzcmi at 15pt % ZapfChancery-MediumItalic 
\font\zapftwenty =pzcmi at 20pt % ZapfChancery-MediumItalic 

\def\emfi#1{{\it #1\/}}		\def\emfs#1{{\sl #1\/}}
\def\emfu#1{\underbar{#1}}	%Underlined emphasis.

%! \ty should be discontinued, it is now \emftt
%! \def\altercatcodes{%
%! %%  Before the following change, the catcodes are:
%! %%\catcode`\@=13  \catcode`\_=8 \catcode`\-=12
%! %%  The change is indeed local to the group; a \begingroup \endgroup does
%! %%  isolate the catcode change.
%!   \catcode`\@=12  \catcode`\_=12 \catcode`\-=12 %
%!   }
%! \def\endgroupafter#1{%
%!   #1%
%!   \endgroup
%!   }
%! \def\emftt{%
%!   \begingroup
%!     \altercatcodes
%!     \tt
%!     \spaceskip.525em plus1.67em minus1.11em %
%!     \xspaceskip1.5em plus1.67em minus1.11em %
%!     \endgroupafter
%!     }
%! \define\fln{\emftt}	%FileName.  Intended also be used for usernames.

%! Work on this
% \def\dofilename#1{%
%   \xdef\filename{#1}%
%   \endgroup
%   }
% \def\setfilename{%
%   \begingroup
%     \altercatcodes
%     \dofilename
%     }
% 

\def\sc{\smc}	% NOTE. This is a \def rather than a \let because the
					% amsppt.sty in its \tenpoint and
					% \eightpoint macros, *re*defines \smc.

\def\st{{$^{\text{\it st}}$}} \def\nd{{$^{\text{\it nd}}$}} \def\th{{$^{\text{\it th}}$}}


  % Font related stuff. (THE STYLE FILE MIGHT CHANGE THESE.)
\def\emf#1{{\it #1\/}}		\def\emff#1{{\bf #1}} % Strong emphasis.
\def\df#1{{\bit #1\/}}		\define\dfw#1{{\bf``}#1{\bf''}} % Weak \df .
\def\thm#1{{\sl #1}}



%! 19jan97 Unfortunately, AMSTeX will break between -- and #1; and putting in \nobreak
%  does not fix the problem.
\def\foreground#1{ --\ignorespaces#1\ignorespaces-- }
%! \def\pc#1{\unskip, \ignorespaces#1\ignorespaces,} %Comma parenthesis.  NOW use
						  %\jc in paren.tex. 


			%%% ENGLISH MACROS %%%
\xdef\monthinwords{\relax
  \ifcase\month
    Month0\or
    January\or
    February\or
    March\or
    April\or
    May\or
    June\or
    July\or
    August\or
    September\or
    October\or
    November\or
    December\else
    Month13
    \fi
  }
\xdef\dateinwords{\monthinwords\ \the\day, \the\year}


% %%%%%%%%%%%%%%%% Catcode changing 
% 	\catcode`\@=11
% 
% 	\catcode`\@=\active
% %%%%%%%%%%%%%%%% End of Catcode changing 


==> my_hyphenations.tex <==
%% To show hyphens:
%% \showhyphens{measurable Borel Baire}
%% \xxx %! This is to find the hyphenation; keep \xxx on a separate line.

% 04Nov97:  TeX appears to have a bug, and (sometimes?) prevents hyphenation
%   of 


  \hyphenation{%
Ber-noulli Pin-sker
dit-to
Lebes-gue
Lem-ma
lem-ma
rough-ly
start-ed
Berg-man
bool-e-an      % I'm not sure that this is correct.  Also, when tested, it
	       % showed bool-ean ??
func-tion-al    % Default is func-tional
dy-a-dic
%! pro-to-brick % IS CORRECTLY HYPHENATED.
%! side-length % IS CORRECTLY HYPHENATED.
%%%% NEW WORDS ARE ABOVE
er-god-ic
an-ti-deriv-a-tive
null-set
Pe-ter-sen
Ak-cog-lu
Roh-lin
pre-print
equi-con-tin-u-ous
sub-in-vari-ant
iso-me-tries
equi-de-com-pos-able
Ox-to-by
Birk-hoff
uni-po-tent
vec-tor-space
equi-dis-tri-bu-tion
de-ter-min-ism
  }



==> standardfonts.ams.tex <==
\ifx\standardfontsLoaded\relax\endinput
\else\global\let\standardfontsLoaded\relax\fi



		%%%%%%%% CHANGES WHICH USE THE @ SYMBOL %%%%%%%%
		\catcode`\@=11

			%%% FONTS %%%
\let\foliofont=\tenbf
\def\itemfont{\sl}

\font@\tenbit=cmbxti10		% For subsection: BOLD TEXT ITALIC.
\font@\eightbit=cmbxti10 at 8pt	% Unfortunately doesn't exist

\font@\eighttt=cmtt8

\font@\zaphtwelve =pzcmi at 12pt % ZapfChancery-MediumItalic
\font@\zaphten =pzcmi at 10pt % ZapfChancery-MediumItalic
\font@\zapheight =pzcmi at 8pt % ZapfChancery-MediumItalic

% Sans serif.		Sans serif italic.
\font@\eightss=cmss8	\font@\eightssi=cmssi8
\font@\tenss=cmss10 	\font@\tenssi=cmssi10

%%%% 19mar96
\font\sevenss=cmss8 at7pt
\font\fivess=cmss8 at5pt

\newfam\ssfam

%! 08Jan98 %  Keep the "\mathchoice", as an example.
% \def\sshack#1{\mathchoice{\hbox{\tenss#1}}{\hbox{\tenss#1}}{\hbox{\sevenss#1}}{\hbox{\fivess#1}}}

  % TEN POINT FONTS
\let\holdtenpoint=\tenpoint
\def\tenpoint{\holdtenpoint
  \textonlyfont@\bit\tenbit
%%%% 19mar96 Start
\textfont\ssfam=\tenss
\scriptfont\ssfam=\sevenss
\scriptscriptfont\ssfam=\fivess
\def\ss{\fam\ssfam \tenss}%
%%%% 19mar96 End
  \textonlyfont@\ssi\tenssi
  }				\tenpoint %Safety.

  % EIGHT POINT FONTS
\let\holdeightpoint=\eightpoint
\def\eightpoint{\holdeightpoint
  \textonlyfont@\bit\eightbit
%%%% 26mar96 Start
\textfont\ssfam=\eightss
\scriptfont\ssfam=\sevenss
\scriptscriptfont\ssfam=\fivess
\def\ss{\fam\ssfam \eightss}%
%%%% 26mar96 End
%!  \textonlyfont@\ss\eightss		%San serif.  \ss is redefined from German es-zet.
  \textonlyfont@\ssi\eightssi
  \baselineskip=10pt
  }
\let\ept=\eightpoint

  % TWELVE POINT FONTS
\font@\twelverm=cmr12
\font@\twelveit=cmti12
\font@\twelvesl=cmsl12
\font@\twelvebf=cmbx12
\font@\twelvesmc=cmcsc10  scaled \magstep1
\font@\twelvett=cmtt12
    % MATH FONTS
\font@\twelvei=cmmi12
\font@\twelvesy=cmsy10   scaled \magstep1
\font@\twelveex=cmex10   scaled \magstep1
\font@\twelvemsx=msxm10  scaled \magstep1

% TWELVEPOINT MACRO
\def\twelvepoint{\def\pointsize@{12}%
%% The values of the next 10 lines (thru \parindent) are stolen from
%%   \tenpoint and are NOT CORRECT.
 \normalbaselineskip 13.333333 pt
 \abovedisplayskip 13.333333 pt plus 3.333333 pt minus 9.999999 pt
 \belowdisplayskip 13.333333 pt plus 3.333333 pt minus 9.999999 pt
 \abovedisplayshortskip 0 pt plus 3.333333 pt
 \belowdisplayshortskip 7.777777 pt plus 3.333333 pt minus 4.444444 pt
 \smallskipamount= 3.333333 pt plus 1.111111 pt minus 1.111111 pt
 \medskipamount=6.666666 pt plus 2.222222 pt minus 2.222222 pt
 \bigskipamount=13.333333 pt plus 4.444444 pt minus 4.444444 pt
 \parskip=2 pt plus 1 pt
 \parindent 16.666666 pt
 \textonlyfont@\rm\twelverm
 \textonlyfont@\it\twelveit
 \textonlyfont@\sl\twelvesl
 \textonlyfont@\bf\twelvebf
 \textonlyfont@\smc\twelvesmc
\ifsyntax@			% This is just to check if the user
				% has put a \syntax command in the
				% source file.  Then, TeX just checks
				% its syntax, more quickly.
%% I DON'T KNOW WHAT THE NEXT TWO LINES SHOULD DO.
%%  \def\big##1{{\hbox{$\left##1\right.$}}}\else
%%  \let\big\tenbig@
 \textonlyfont\z@\twelverm  \scriptfont\z@\tenrm  \scriptscriptfont\z@\eightrm
 \textonlyfont\@ne\twelvei  \scriptfont\@ne\teni  \scriptscriptfont\@ne\eighti
 \textonlyfont\tw@\twelvesy \scriptfont\tw@\tensy \scriptscriptfont\tw@\eightsy
 \textonlyfont\thr@@\twelveex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
 \textonlyfont\itfam\twelveit
 \textonlyfont\slfam\twelvesl
 \textonlyfont\bffam\twelvebf \scriptfont\bffam\tenbf
   \scriptscriptfont\bffam\eightbf
 \textonlyfont\msxfam=\twelvemsx  \scriptfont\msxfam=\tenmsx
   \scriptscriptfont\msxfam=\eightmsx
 \textonlyfont\msyfam=\twelvemsy
   \scriptfont\msyfam=\tenmsy
   \scriptscriptfont\msyfam=\eightmsy
 \fi
%% \setbox\strutbox\hbox{\vrule height8.5\p@ depth3.5\p@ width\z@}%
%% \setbox\strutbox@\hbox{\vrule height8\p@ depth3\p@ width\z@}%
 \normalbaselines\twelverm\ex@=.2326ex}	% The value for \ex@ here is
				       	% that stolen from \tenpoint
				       	% and are NOT CORRECT.
			\catcode`\@=\active


==> stylechanges.ams.tex <==
% This is par of jk.sty I am using to try to run with
% version 2 of AMSTEX.
% THIS IS NOT A COMPLETE STYLE FILE!  This is to be \input AFTER amsppt.sty is loaded.

% Projects:

\ifx\stylechangesLoaded\relax\endinput
\else\global\let\stylechangesLoaded\relax\fi

    \ifx\everytexLoaded\relax
    \else\input everytex.tex\fi

    \ifx\standardfontsLoaded\relax
    \else\input standardfonts.ams.tex\fi

    \input my_hyphenations.tex

% 15Jul1998:  Moved \cn (call number) to "everytex.tex".

	\catcode`\@=11


\TagsOnRight
%%%% \hsize \vsize
\hcorrection{-.3truein}	\pagewidth{7.1truein}

% \vcorrection{-.25truein} % This value works fine for printing, but not for previewing.
                           % When I run xdvi on the .dvi file, the header is not visible
			   % and cannot be made visible.
\vcorrection{.29truein} 
\pageheight{9.00truein}	%\pageheight{9.15truein}

\let\logo@=\relax %This kills off the annoying logo.  Someday I should rewrite
		  %this so that it is optional.   KEEP THIS, in case \output is changed.

\def\foliofont@{\tenbf}
\def\headlinefont@{\eightpoint\it}
\def\proclaimfont{\sl}
\def\proclaimheadfont@{\smc}
\def\demofont@{\smc}


%%%%%%%%%%%%%%%% HEADLINE Stuff %%%%%%%%%%%%%%%%

%jk: I've removed the "\frills@\uppercasetext@" from each
%  of the following definitions.
\def\leftheadtext{\let\savedef@\leftheadtext
  \def\leftheadtext##1{\let\leftheadtext\savedef@
    \leftheadtoks\expandafter{{##1}}%
    \mark{\the\leftheadtoks\noexpand\else\the\rightheadtoks}
    \ifsyntax@\setboxz@h{\def\\{\unskip\space\ignorespaces}%
        \headlinefont@##1}\fi}%
  \nofrillscheck\leftheadtext}

\def\rightheadtext{\let\savedef@\rightheadtext
  \def\rightheadtext##1{\let\rightheadtext\savedef@
    \rightheadtoks\expandafter{{##1}}%
    \mark{\the\leftheadtoks\noexpand\else\the\rightheadtoks}%
    \ifsyntax@\setboxz@h{\def\\{\unskip\space\ignorespaces}%
        \headlinefont@##1}\fi}%
  \nofrillscheck\rightheadtext}

%% IN AmsTeX2, \rightheadline and \leftheadline have now become token sequences.
\rightheadtext{\titlename}  \def\titlename{NO TITLE}	% SAFETY
\leftheadtext{J.L.\,King}



%%%%%%%%%%%%%%%% FOOTLINE Stuff %%%%%%%%%%%%%%%%

\def\nofootline{\global\footline{\hfil}}
\define\setupfootline{\global\footline={\eightpoint\ssi
      \ifodd\pageno\rightfootline \else\leftfootline\fi}}

%% IMPORTANT: \touchdate and \filename are to be set in the user file.
\def\footlineweb{%
  \hfil
  Some jk articles available at webpage:~{\ss http://www.math.ufl.edu/$\sim$squash/}%
  \hfil
  }
%
\def\footlinedate{%
  As of: \touchdate%
  \hfil
  Typeset: {\ss \dateinwords}%
  }
%
\def\footlinefilename{%
  \hfil
  Filename is {\tt \filename}%
  \hfil
  }
%
\def\footlinefilenameanddate{%
  Typeset: {\ss \dateinwords}%
  \hfil
  Filename is {\tt \filename}%
  }
%
\def\footlinefilenameandtouchdate{%
  Filename is {\tt \filename}%
  \hfil
  As of: \touchdate.%
  }
%
%! \def\footlinefilenamethendate{%
%!   \footlinefilename
%!   \glet\rightfootline=\footlinedate
%!   \glet\leftfootline=\footlinedate
%!   }
%
\def\footlinewebthenrightdate{%
  \footlineweb
  \glet\rightfootline=\footlinedate
  }
% 
\def\footlinedatefilenametouchdate{%
  Typeset: {\ss \dateinwords}%
  \hfil
  Filename: {\tt \filename}%
  \hfil
  As of: \touchdate%
  }


% INTIALIZATION
\setupfootline
\let\rightfootline=\footlinedatefilenametouchdate
\let\leftfootline=\footlinedatefilenametouchdate
\def\filename{NoFile} \def\touchdate{NoDate} %Safety


%%%%%%%%%%%%%%%% OUTPUT %%%%%%%%%%%%%%%%
%Redefine \output to allow simultaneous headlines and footlines.

%%% This is from amsppt.sty (presumably, one designed for AMSTEX version 2)
% The changes are on separate lines.
\def\output@{\shipout\vbox{%
 \iffirstpage@ \global\firstpage@false
  \pagebody
  %CHANGES The  \logo@  has been deleted
  \makefootline%
 \else \ifrunheads@ \makeheadline \pagebody
       \makefootline %CHANGES The footline has been added.
       \else \pagebody \makefootline \fi
 \fi}%
 \advancepageno \ifnum\outputpenalty>-\@MM\else\dosupereject\fi}


\catcode`\@=\active

%%%%%%%%%%%%%%%% Style changes %%%%%%%%%%%%%%%%
% There appears to be something wrong with the amsppt.sty version of \demo, in amstex2.  I
% don't now recall what the problem was.
%! The following needs to be rewritten

%! \def\demo#1{\medbreak\smallskip
%!   \noindent{\sc #1.}\hskip8pt plus6pt minus4pt\ignorespaces
%!   }
%! \def\enddemo{\relax}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%% \enddocument Stuff %%%%%%%%%%%%%%%%
%
% NB:  I can tokens to \enddocument so that it changes the \footline for the
% last page, if desired.
%
\toks0=\expandafter{\enddocument}
% 
% \edef\enddocument{\nobreak\bigskip
%   {\noindent\noexpand\ept Filename is:\par
%   \noindent\hskip20pt minus20pt\noexpand\tt \noexpand\filename\par} \the\toks0}

\edef\enddocument{\nobreak\bigskip
 { %! The following 2 lines, redefining the footline, appear to work -but I
   %  don't fully know why they work.  Currently, I don't use them.
   %
  %!
 \noexpand\setupfootline
  %
 \noexpand\global\noexpand\let\noexpand\rightfootline\noexpand=\noexpand\footlineweb
  %
 \noexpand\global\noexpand\let\noexpand\leftfootline\noexpand=\noexpand\footlineweb
  %
  \noexpand\ept
  {\noindent Filename is:%
    \penalty0\hbox{}\nobreak\hskip 20pt minus15pt%
    {\noexpand\tt \noexpand\filename}\par}%
  % 
  {\noindent As of: %
    {\noexpand\sl \noexpand\touchdate}%
    \quad Typeset: %
    {\noexpand\sl \noexpand\dateinwords}\par}% 
  }% 
  \the\toks0}
% 
%%%%%%%%%%%%%%%% STOP \enddocument Stuff %%%%%%%%%%%%%%%%

